Benchmarking Contextual Understanding for In-Car Conversational Systems

In-Car Conversational Question Answering (ConvQA) systems significantly enhance user experience by enabling seamless voice interactions. However, assessing their accuracy and reliability remains a challenge. This paper explores the use of Large Language Models (LLMs) alongside advanced prompting techniques and agent-based methods to evaluate the extent to which ConvQA system responses adhere to user utterances. The focus lies on contextual understanding and the ability to provide accurate venue recommendations considering user constraints and situational context. To evaluate utterance-response coherence using an LLM, we synthetically generate user utterances accompanied by correct and modified failure-containing system responses. We use input-output, chain-of-thought, self-consistency prompting, and multi-agent prompting techniques with 13 reasoning and non-reasoning LLMs of varying sizes and providers, including OpenAI, DeepSeek, Mistral AI, and Meta. We evaluate our approach on a case study involving restaurant recommendations. The most substantial improvements occur for small non-reasoning models when applying advanced prompting techniques, particularly multi-agent prompting. However, reasoning models consistently outperform non-reasoning models, with the best performance achieved using single-agent prompting with self-consistency. Notably, DeepSeek-R1 reaches an F1-score of 0.99 at a cost of 0.002 USD per request. Overall, the best balance between effectiveness and cost-time efficiency is reached with the non-reasoning model DeepSeek-V3. Our findings show that LLM-based evaluation offers a scalable and accurate alternative to traditional human evaluation for benchmarking contextual understanding in ConvQA systems.

==> chapters/future_work.tex <==
% !TEX root =  main.tex
\section{Future Work}
% \label{sec:future-work}

\Lev{Merge with conclusion}

% This study establishes a foundation for evaluating in-car \ac{convqa} systems by focusing on contextual understanding.

% Future research can build on this by extending the evaluation to several key areas and explore its application in other domains, such as assisting with the owner’s manual or addressing car functionality queries.
% Expanding into these areas would allow testing of the system adaptability across various in-car scenarios. 

% In this study we have evaluated LLM-based judgment on restaurant-related recommendations. To provide a more comprehensive assessment, future work could include other places of interests, such as gas stations, electric vehicle chargers, or grocery stores. 
% It would be also interesting to understand whether our findings apply also for recommendations in other languages which is in particular important when deploying vehicles in different countries.

% Moreover, increasing the complexity of human-machine interactions by incorporating multi-turn conversations, rather than single-turn queries, would offer deeper insights into the ability to manage context understanding over extended dialogues.
% Furthermore, the class imbalance in the dataset of contextual understanding, where positive cases (N=100) were fewer than negative ones (N=500), likely influenced the F1-Score.
% Future work should use a more balanced dataset, to address this limitation and improve the robustness of evaluations.
% Next, with the rapid advancement of \acp{llm}, future studies should regularly incorporate newer models, to ensure that benchmarking efforts remain current with AI developments.
% Testing a broader range of models and agentic methods, as well as experimenting with newer prompting strategies, could yield further improvements in \ac{llm} performance.
% Evaluating these models in different languages would also ensure that the system performs well across multilingual environments, an essential factor for global deployment. 
Besides that, increasing the complexity of interactions by incorporating multi-turn conversations, rather than single-turn queries, would offer deeper insights into the ability to manage context understanding over extended dialogues.

% Expanding the dataset size and diversity would allow for more rigorous testing, helping to uncover potential limitations.

% Finally, future research should emphasize real-world testing of these systems, ensuring their effectiveness under varied and complex conditions to guarantee reliability and safety in practical applications.



==> chapters/other-chapters.tex <==
% !TEX root =  main.tex
\section*{Author Contributions}\label{sec:author-contributions}


% see https://www.sciencedirect.com/journal/journal-of-systems-and-software/publish/guide-for-authors
% Author contributions: CRediT
\textbf{Philipp Habicht:} Methodology, Software, Validation, Formal Analysis, Data curation, Visualization, Writing - Original draft
\textbf{Lev Sorokin:}
\textbf{Abdullah Saydemir:} Software, Validation, Formal analysis, Visualization, Writing - Review \& Editing
\textbf{Ken Friedl:}
\textbf{Andrea Stocco:}
